Formulating or Fixating: Effects of Examples on Problem Solving Vary as a Function of Example Presentation Interface Design

Interactive systems that facilitate exposure to examples can augment problem solving performance. However designers of such systems are often faced with many practical design decisions about how users will interact with examples, with little clear theoretical guidance. To understand how example interaction design choices affect whether/how people benefit from examples, we conducted an experiment where 182 participants worked on a controlled analog to an exploratory creativity task, with access to examples of varying diversity and presentation interfaces. Task performance was worse when examples were presented in a list, compared to contextualized in the exploration space or shown in a dropdown list. Example lists were associated with more fixation, whereas contextualized examples were associated with using examples to formulate a model of the problem space to guide exploration. We discuss implications of these results for a theoretical framework that maps design choices to fundamental psychological mechanisms of creative inspiration from examples.

==> cutting-room-floor.tex <==
%Interactive systems that facilitate exposure to examples have potential to augment designers' creative performance. We think this because past research has hypothesized that exposure to diverse examples could help individuals come up with more diverse and creative ideas \cite{gentnerStructureMappingAnalogy1997, holyoakMentalLeapsAnalogy1995, pozeAnalogicalConnectionsEssence1983, wardAnalogicalDistancePurpose1998, eckertFortuneFavoursOnly1998}. Moreover, there is both empirical evidence \cite{leeDesigningInteractiveExample2010, dahlInfluenceValueAnalogical2002, atkinsonLearningExamplesInstructional, schon1985design, siangliulueProvidingTimelyExamples2015} and anecdotal facts \cite{findlayHundredYearsChemistry1965, freeman1997didn, kalogerakisDevelopingInnovationsBased2010} for this hypothesis.

%But we don't have a theory that can directly inform these design decisions. Prior theories of the effects of examples can speak to how variations in levels of diversity influence the creative process and outputs, but their level of description does not provide adequate guidance for these interaction design decisions. For example, there is a lot of research on conceptual combination in psychology, but the majority of that work focuses on pairs of examples only \cite{gentnerStructureMappingAnalogy1997, holyoakMentalLeapsAnalogy1995, pozeAnalogicalConnectionsEssence1983, wardAnalogicalDistancePurpose1998}, and so cannot speak to situations where interaction design decisions about screen size may come in, such as with a larger number of examples. On the flip side, there is a lot of empirical work on different example interfaces in HCI \cite{xuIdeateRelateExamplesGallery2021, macneilProbMapAutomaticallyConstructing2021, odonovanDesignScapeDesignInteractive2015, wangIdeaExpanderSupporting2010a, andolinaInspirationWallSupportingIdea2015, changRecipeScapeInteractiveTool2018, pavelBrowsingAnalyzingCommandLevel, kellerCollectingCabinetHow2009, mendelsFreedSystemCreating2011, ivanovMoodCubesImmersiveSpaces2022}, but little integration across the studies into a coherent theory. Therefore, we hope to fill in the theoretical gap of whether and how example interaction design choices might influence the degree to which people benefited from diverse examples. This prompts us to ask two research questions (RQs):

%Designers often use others’ work as examples to inspire their own work in the design field \cite{atkinsonLearningExamplesInstructional, herringGettingInspiredUnderstanding2009, xuIdeateRelateExamplesGallery2021, schon1985design, siangliulueProvidingTimelyExamples2015, yenSeekingExemplarsWild2022}. Kulkarni et al. \cite{kulkarniEarlyRepeatedExposure2012} showed that early exposure to examples improves designers’ creativity and repeated exposure to examples interspersed with prototyping leads to even better results. One basic reason for the improvement is that examples can directly shape ideation by providing features or conceptual elements to use, or offering a direction of thinking. For instance, when undergraduate students drew imaginary animals, typical features from earth animals were frequently included, with occasional deviations \cite{wardStructuredImaginationRole1994}. Another concrete evidence is that examples' features can shape ideation by shaping what other ideas are available, through spreading activation \cite{collinsSpreadingactivationTheorySemantic1975} and priming \cite{mcnamaraPrimingConstraintsIt1992}.
%However, when features get transferred over directly from examples whether we want it to or not, examples could also cause fixation \cite{janssonDesignFixation1991, marshConceptualPrimingGenerative1999, marshInadvertentUsePrior1999, perttulaIdeaExposureParadigm2007, smithConstrainingEffectsExamples1993}. Sometimes this feature transfer happens without conscious awareness of having done so \cite{linseyStudyDesignFixation2010, dowCheatersNeverProsper2015}. This fixation effect may also be referred to as cryptomnesia \cite{marshItemAvailabilityCryptomnesia1995}, conformity effect \cite{perttulaExposureEffectsDesign2006}, and structured imagination \cite{wardStructuredImaginationRole1994} in psychological studies. Fixation is reflected in various ways, for example, new designs often share features of examples after seeing an example concept even with its flaws pointed out \cite{janssonDesignFixation1991}; and people find it very difficult to see an objects with well known uses can be applied in new or unusual ways to develop an innovative solution \cite{purcellDesignOtherTypes1996}. Those fixations are due to some knowledge about existing or obvious solutions being spontaneously activated and constraining the ideation of new solutions \cite{agogueImpactTypeExamples2014}.

%, including design recommendation \cite{siangliulueProvidingTimelyExamples2015, kochMayAIDesign2019, wangIdeaExpanderSupporting2010a, andolinaInspirationWallSupportingIdea2015, chanSemanticallyFarInspirations2017, kochImageSenseIntelligentCollaborative2020}, searching for examples and stimuli \cite{macneilProbMapAutomaticallyConstructing2021, kochImageSenseIntelligentCollaborative2020}, explorable overviews \cite{xuIdeateRelateExamplesGallery2021, changRecipeScapeInteractiveTool2018, pavelBrowsingAnalyzingCommandLevel}, integration with ideation workspace \cite{kochImageSenseIntelligentCollaborative2020, kochSemanticCollageEnrichingDigital2020, ivanovMoodCubesImmersiveSpaces2022, kellerCollectingCabinetHow2009, sharminReflectionSpaceInteractiveVisualization2013, sharminUnderstandingKnowledgeManagement2009b, mendelsFreedSystemCreating2011} and example dissection \cite{changWebCrystalUnderstandingReusing2012, siangliulueCollaborativeIdeationScale2015, siangliulueIdeaHoundImprovingLargescale2016, kumarBricolageExamplebasedRetargeting2011, wangInterpretableDirectedDiversity2022}.

==> sections/3-theory.tex <==
% NOT USED %

\section{Theoretical Framework}

We would like our \theory{} to bridge two strands of literature: 1) basic studies and theories of inspiration from examples, with careful attention to the mechanisms of action, and 2) proposals for systems for interacting with examples to support creative work. The former literature consists of the theoretical and experimental psychological literature on creativity, as well as studies of design practice (often in an ethnographic tradition). The latter literature is situated primarily in the HCI literature, along with cognate fields that create new creativity support artifacts that target working with examples, such as case-based reasoning and decision-support systems.

We frame our bridging of these strands of literature based on an influential family of models in design theory that model design as a process of constructing connections between three different aspects of a design object: 1) its \textbf{function} - what it is for, 2) its \textbf{behavior(s)} - what it does, and 3) its \textbf{structure} - what it is (e.g, its components and their interrelationships). One of the most influential of these models is Gero's Function-Behavior-Structure framework \cite{geroDesignPrototypesKnowledge1990,geroSituatedFunctionbehaviourstructureFramework2004}, but there are important variants such as Goel's Structure-Behavior-Function (SBF) model \cite{goelStructureBehaviorFunction2009}. These models are useful in design practice and theory for modeling design problems and processes; here, we find it useful as a framework to bridge between fundamental theories and studies, which can articulate desired \textit{functions} of interfaces for interacting with examples, and key design decisions about the \textit{structure(s)} of artifacts and designs for such interfaces. The \textit{behavior(s)} that mediate interactions between structure and function can be thought of as the desired affordances of the system.

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/examples-interaction-theory_v0.png}
    \caption{Overview of mapping between functional outcomes and behavioral affordances of working with examples. Each mapping is a hypothesized "unlocks" relation: for example, enabling designers to analyze examples unlocks repurposing functions, and enabling designers to contextualize examples unlocks modeling functions.}
    \label{fig:theory-figure}
\end{figure}

\subsection{Overview}
Figure X shows an overview of our framework. From the literature, we synthesize four levels of functional outcomes of examples that can lead to creative inspiration: in ascending order of sophistication, these are 1) priming, 2) repurposing, 3) combination and integration, and 4) modeling. These levels of functional outcomes are then mapped to four key behaviors of working with examples: 1) viewing, 2) analyzing, 3) comparing, and 4) contextualizing. The intuition behind this mapping is that each of these behaviors "unlocks" a particular level of functional outcome: for example, enabling analysis behavior unlocks the functional outcome of repurposing (simply viewing is insufficient), and enabling comparison behaviors unlocks the functional outcomes of combination and integration.

We first describe each of these functional outcomes, discussing their grounding in the literature. Next, we describe the behaviors, and their mapping to functional outcomes. We then describe examples of interfaces (structures) that support different combinations of these behaviors. Finally, we demonstrate how the framework generates predictions for the functional outcomes of those interfaces w.r.t. the use of examples and their impact on ideation.

\subsection{Levels of functional outcomes from examples}
Let's first consider the key functional outcomes of examples for creative ideation: in other words, what we expect to happen from a specific creative cognition perspective, rather than interface-oriented behaviors.

\subsubsection{Stimulate}
The most basic functional outcome is that examples can directly shape ideation by providing features or conceptual elements to use, or priming a direction of thinking. \todo{Examples of this include...}

The foundation for this functional outcome is a robust set of results from experimental studies of creative cognition that show how, when exposed to examples, people very frequently transfer features from the examples into their ideas \cite{smithConstrainingEffectsExamples1993,wardStructuredImaginationRole1994,dowCheatersNeverProsper2015}. Sometimes this feature transfer happens without conscious awareness of having done so \cite{linseyStudyDesignFixation2010,dowCheatersNeverProsper2015}, a phenomenon known in psychological research as cryptomnesia. This feature transfer effect is quite frequently so strong that it happens despite instructions to avoid such transfer \cite{marshInadvertentUsePrior1999,janssonDesignFixation1991,georgeConstrainingConstructiveEffects2017}, and is not entirely ameliorated by design expertise \cite{linseyStudyDesignFixation2010,dowCheatersNeverProsper2015}. 

This feature transfer is often discussed in negative terms as "conformity" (see, e.g., \cite{smithConstrainingEffectsExamples1993}), "structured imagination" \cite{wardStructuredImaginationRole1994}, or even "fixation" \cite{janssonDesignFixation1991}. This is not unsurprising, since a typical result is high similarity between the example and the idea. However, what is important to note here is not that examples overall have a positive or negative effect on creative performance, but rather that they can stimulate exploration in a particular direction. Whether that ends up being positive or negative is dependent on the particulars of the task and example, and the relationship between the two. For instance, when the example is an idea that is novel to some domain \textit{and} likely to solve the problem in that domain in an important way, then direct stimulation of an exploration direction will have a positive effect on creative performance. This is the argument made by \cite{purcellDesignOtherTypes1996}, and corroborated in some empirical studies that show positive results on novelty and/or quality despite --- or perhaps because of --- transferring features from examples \cite{marshHowExamplesMay1996,georgeConstrainingConstructiveEffects2017,agogueImpactTypeExamples2014}; often this is tied to the originality/creativity of the examples, whether transferring features from more creative examples leads to more creative ideas. 

A related set of results concerns the idea of \textbf{priming} from examples \cite{mcnamaraPrimingConstraintsIt1992}. Here, in addition to shaping ideation by directly transferring features, examples can also shape what concepts are activated in memory and available for use for ideation. The principal explanation for this effect is spreading activation \cite{collinsSpreadingactivationTheorySemantic1975} from the example as a cue, to other related concepts in memory, making them more available; but there is some controversy over the detailed mechanics of this theoretical explanation \cite{ratcliffDoesActivationReally1981}. The Search in Associative Memory (SIAM) model of ideation was originally proposed to apply this theory to the context of group ideation, to account for whether/how exposure to ideas from others leads to net ideation gains; a key component of the model describes ideas from others as enabling people to generate more ideas, often by searching more deeply within categories, by activating additional ideas in memory through spreading activation \cite{nijstadHowGroupAffects2006}. Consistent with this model several experiments have found stimulation effects in terms of number, and sometimes variety of ideas, via exposure to ideas of others \cite{nijstadHowGroupAffects2006,kordeAlternatingIndividualGroup2016,yagolkovskiyEnhancementCreativitySemantic2020}

Overall, the functional outcome of stimulation from examples can be quite positive. However, because of the dynamics of spreading activation and priming, there is an upper bound on performance if the task requires substantial diversity of ideas or significant departures from the examples. This leads to the next functional outcome of working with examples: repurposing.

\subsubsection{Repurpose}
The second outcome --- repurposing --- is similar to stimulating, but goes a step further: rather than transferring all or most of the elements of an example, this outcome involves taking particular elements from the example and using it in a new idea in a way that departs significantly from the example.

For instance, consider... \todo{Examples of this include...}

This can be seen in a number of studies that followed up on the conformity effect observed above, in attempts to discover conditions under which people were not only able to avoid worse creative outcomes of novelty or quality, but also fixation on features of the examples. For instance, \cite{okadaImitationInspirationCreation2017} found that artists who copied . Similarly, Mecca and colleagues found that people who used more advanced "propulsion strategies" when working with examples, such as redefining an exemplar concept from an alternative perspective, generated more high quality and novel ideas than people who simply replicated or imitated the examples wholesale \cite{meccaImitationCreativityBeneficial2013}.  A related finding is that inducing or providing a higher level problem schema with examples enables analogical transfer of a solution principle from one domain to another that seems unrelated on the surface \cite{}. 

Studies of example use by expert designers also bear this out. For example, 

The core idea here of adaptation or repurposing is supported by a number of core cognitive processes. One of these is abstraction. 

The common thread across these findings is that participants are gaining additional benefits from examples and/or avoiding potentially negative effects of fixation, by repurposing partial features

People induce higher-level principles or emergent features from the examples, which then guide or influence ideation in ways that can depart significantly from the original example(s). 

This is also consistent with studies of analogical transfer and outsider innovation and knowledge brokering, where good ideas are transferred from one domain to another to inspire new creative breakthroughs.

\subsubsection{Combine and integrate}
The next functional outcome of integrating builds on the previous ones: rather than transferring or repurposing elements from a single example, this outcome combines or integrates elements from multiple examples into a new whole. Often this new whole is greater than the sum of its parts, with emergent properties of the whole that are not true of its parts.

\todo{Examples of this include...}

\todo{The lit on this includes...}

\subsubsection{Model}
Finally, we have the functional outcome of modeling. Here, there is a greater distance between the specific features of examples and what ideas result: rather than serving as stimulation, or sources of specific features to transfer or recombine, the examples are used to induce a higher level model of one or more relevant design spaces, problem formulations, or frames, which then guides exploration.

\todo{Examples of this include...}

\todo{The lit on this includes...}
The literature on this comes moreso from research in a more qualitative and ethnographic tradition, rather than experimental, focusing on developing theory from \textit{in situ} observations of creative practice with examples.

The core idea here is that the examples here are used for more than solution elements; they interact in intricate ways with the designers' formulation, or model, of the problem. They are used to get a higher level sense of promising directions, the shape of the space, and sometimes even to trigger and support reformulation of the problem itself.

\subsection{From Behavioral Affordances of Working with Examples to Functional Outcomes of Examples}
Let's now consider how the aforementioned functional outcomes might map to specific observable behaviors that are closer to the way that designers reason about the effects of their interfaces.

\subsubsection{View}
View is simplest. No affordances for doing anything more with examples. Typical in most experiments. Not often seen in HCI; this is where interactive systems have potential, to let us do more with examples than manipulate what they are, or instructions!

\subsubsection{Analyze}


\subsubsection{Compare}

\subsubsection{Contextualize}

% A critical feature of our framework is the ordering of functions in levels of sophistication in terms of interactions with examples.

% Basic processes that are hypothesized, theorized and observed.

% Practices that emerge in expert practice and interactions with examples.

% Predictions:
% - Systems for interacting with examples that only enable people to view, will have limited impact on ideation; at most, priming in a different direction, which is useful under specific circumstances (e.g., being especially fixated).
% - 
